An on-demand resource allocation algorithm for a quantum network hub and its performance analysis

To effectively support the execution of quantum network applications for multiple sets of user-controlled quantum nodes, a quantum network must efficiently allocate shared resources. We study traffic models for a type of quantum network hub called an Entanglement Generation Switch (EGS), a device that allocates resources to enable entanglement generation between nodes in response to user-generated demand. We propose an on-demand resource allocation algorithm, where a demand is either blocked if no resources are available or else results in immediate resource allocation. We model the EGS as an Erlang loss system, with demands corresponding to sessions whose arrival is modelled as a Poisson process. To reflect the operation of a practical quantum switch, our model captures scenarios where a resource is allocated for batches of entanglement generation attempts, possibly interleaved with calibration periods for the quantum network nodes. Calibration periods are necessary to correct against drifts or jumps in the physical parameters of a quantum node that occur on a timescale that is long compared to the duration of an attempt. We then derive a formula for the demand blocking probability under three different traffic scenarios using analytical methods from applied probability and queueing theory. We prove an insensitivity theorem which guarantees that the probability a demand is blocked only depends upon the mean duration of each entanglement generation attempt and calibration period, and is not sensitive to the underlying distributions of attempt and calibration period duration. We provide numerical results to support our analysis. Our work is the first analysis of traffic characteristics at an EGS system and provides a valuable analytic tool for devising performance driven resource allocation algorithms.

==> figs/CompareOpModes.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{p{0.7in}||p{1.0in}|p{2.0in}|p{1.0in}}
        \textbf{Feature} &  \textbf{Operation Mode} & \textbf{Description} & \textbf{Sample \newline Parameters}\\
        \hline
        Maximum \newline attempt rate  & Heralded \newline Entanglement \newline Generation & Limited by the RTT time. The heralding flag must arrive before initiating a subsequent attempt & 9259 attempts/s\\
        \hline
        & Correlated \newline Information \newline Generation & Set by the maximum emission rate of a photonic client & 200 MHz \\
        \hline
        
    \end{tabular}
    \caption{Caption}
    \label{tab:compareOpModes}
\end{table}

==> figs/NonUniformParams.tex <==
\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
        \textbf{Description} &  \textbf{Value} \\
        \hline
        Link lengths, set 1: users $1 - \lceil K/2 \rceil $ & 10 km  \\
        Link lengths, set 2: users $ (\lceil K/2 \rceil  + 1) -  K $ & 20 km  \\
        Single-mode optical fiber attenuation coefficient, $\sigma_{\text{att}}$ & 0.2 \ dB/km \\
        One-way communication time, $S_2$ (\text{RTT}/2) & 100.07 $\mu$s \\
        % Buffer for jitter in heralding flag arrival, set 2 &  20.008   $\mu$s \\
        Resource allocation duration, $S_1$ & 125 ms \\
        Resource allocation duration, $S_2$ & 240 ms \\
        Probability photon travelling 1 km optical fiber arrives, $p_a = {10^{-(\sigma_{\text{att}} / 10)}}$ & 0.95499 (a.u.) \\
        Probability of single attempt success, set 2, $p_{\text{gen}} \cdot p^{20}_{a} / p^{10}_{a}$ & 6.31e-6 (a.u.)\\
        Duration of a single attempt, $S_2$ & 230.146 $\mu$s\\ 
    \end{tabular}
    \caption{Additional physical parameter settings for a non-homogeneous traffic scenario where half of the nodes have doubled link lengths to the EGS.
    These parameters supplement those of Table \ref{tab:sampleParams}.}
\label{tab:nonUniformParams}
\vspace{-5mm}
\end{table}

==> figs/OldParamTable.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Relevance} & \textbf{Description} &  \textbf{Value} \\
        \hline
        General & Link lengths & 10 km  \\
        General & Optical Switching time & 1 ms\\ 
        General & One-way communication time (\text{RTT}/2) & 50.03 $\mu$s \\
        General & Buffer for jitter in heralding flag arrival ($0.1 \times \text{RTT}/2$) &  5.003   $\mu$s \\
        General & Resource allocation duration & 125 ms \\
        \hline
        HE Protocol & Duration of BSM & 10 $\mu$s \\
        HE Protocol & Duration of CR check & 1 ms \\
        HE Protocol & Probability of single attempt success, $p_{\text{gen}}$ & 1e-5 (dimensionless)\\
        HE Protocol & Duration of a single attempt & 115.066 $\mu$s\\ 
        HE Protocol & Maximum attempt rate & 8000 attempts/s \\
        HE Protocol & Number attempts per resource allocation period & 1000 \\
        \hline
        CI Protocol & Probability of single attempt success, $p^{\text{CI}}_{\text{succ}}$ & 0.1156 (dimensionless) \\ 
        CI Protocol & Duration of a single attempt & 50.03  $\mu$s \\
        CI Protocol & Maximum attempt rate & 200 MHz \\
        CI Protocol & Number attempts per resource allocation period & 21 999 065
    \end{tabular}
    \caption{Sample physical parameter values dictating the operation of an EGS. These parameters settings are used in the simulations used in the Numerical Evaluations of Section \ref{sec:NumEval}.}
    \label{tab:sampleParams}
\end{table}
